CoPL: Collaborative Preference Learning for Personalizing LLMs

Personalizing large language models (LLMs) is important for aligning outputs with diverse user preferences, yet existing methods struggle with flexibility and generalization. We propose CoPL (Collaborative Preference Learning), a graph-based collaborative filtering framework that models user-response relationships to enhance preference estimation, particularly in sparse annotation settings. By integrating a mixture of LoRA experts, CoPL efficiently fine-tunes LLMs while dynamically balancing shared and user-specific preferences. Additionally, an optimization-free adaptation strategy enables generalization to unseen users without fine-tuning. Experiments on UltraFeedback-P demonstrate that CoPL outperforms existing personalized reward models, effectively capturing both common and controversial preferences, making it a scalable solution for personalized LLM alignment. The code is available at https://github.com/ml-postech/CoPL.

==> table/ablation_expert_num.tex <==
% \begin{table}[t]
% \centering

% \begin{tabular}{lcc}
% \toprule
%  & UF-P-2-ALL & UF-P-4-ALL \\
% \midrule
% 2  & $63.17_{\pm0.19}$ & $62.56_{\pm0.31}$ \\
% 4  & $63.37_{\pm0.15}$ & $62.68_{\pm0.48}$ \\
% 8  & $63.81_{\pm0.16}$ & $62.57_{\pm0.38}$ \\
% 16 & $63.26_{\pm0.49}$ & $62.58_{\pm0.52}$ \\
% \bottomrule
% \end{tabular}

% \caption{Ablation study of \textbf{CoPL} on \texttt{gemma-2b-it}: accuracy (\%) for UF\,+\,P–2–ALL and UF\,+\,P–4–ALL while varying the number of experts. Results are reported as mean $\pm$ standard deviation over three random seeds.}
% \label{tab:ablation_expert_num}
% \end{table}






==> table/acc_reward_model_tldr.tex <==
% \begin{table*}[t!]
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{llccccc}
% \toprule
% && \multicolumn{2}{c}{\texttt{Gemma-2b-it}} & \multicolumn{2}{c}{\texttt{Gemma-7b-it}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6}
% & & ALL & AVG & ALL & AVG \\
% \midrule 
% \multirow{7}{*}{%
%     \rotatebox[origin=c]{90}{%
%         \parbox{1.3cm}{\centering \emph{Seen}}%
%     }%
% }    
% & Oracle     
% & $73.06_{\pm0.23}$ & $73.06_{\pm0.23}$ & $77.21_{\pm0.28}$ & $77.21_{\pm0.28}$ \\
% \cmidrule(lr){2-6}
% & Uniform    
% & $49.62_{\pm0.09}$ & $49.62_{\pm0.09}$ & $49.39_{\pm0.52}$ & $49.39_{\pm0.52}$ \\
% & I2E        
% & $49.93_{\pm0.23}$ & $49.74_{\pm0.06}$ & $49.40_{\pm0.77}$ & $49.66_{\pm0.31}$ \\
% & I2E$_{\text{proxy}}$
% & $49.80_{\pm0.16}$ & $49.54_{\pm0.13}$ & $49.50_{\pm0.73}$ & $49.95_{\pm0.34}$ \\
% & VPL        
% & $49.52_{\pm0.14}$ & $49.44_{\pm0.21}$ & $49.14_{\pm0.72}$ & $49.17_{\pm0.67}$ \\
% & PAL        
% & $50.12_{\pm0.13}$ & $50.15_{\pm0.15}$ & $49.57_{\pm0.09}$ & $49.75_{\pm0.27}$ \\
% & \ours{}
% & $\textbf{96.58}_{\pm0.09}$ & $\textbf{96.19}_{\pm0.02}$ & $\textbf{97.85}_{\pm0.07}$ & $\textbf{97.88}_{\pm0.01}$ \\
% \midrule \midrule
% \multirow{7}{*}{%
%     \rotatebox[origin=c]{90}{%
%         \parbox{1.3cm}{\centering \emph{Unseen}}%
%     }%
% }    
% & Oracle     
% & $72.55_{\pm1.79}$ & $72.55_{\pm1.79}$ & $77.54_{\pm0.49}$ & $77.54_{\pm0.49}$ \\
% \cmidrule(lr){2-6}
% & Uniform    
% & $50.11_{\pm0.36}$ & $50.11_{\pm0.36}$ & $49.03_{\pm0.76}$ & $49.03_{\pm0.76}$ \\
% & I2E        
% & $49.85_{\pm0.38}$ & $49.16_{\pm0.82}$ & $49.64_{\pm0.98}$ & $49.56_{\pm0.49}$ \\
% & I2E$_{\text{proxy}}$
% & $49.75_{\pm0.94}$ & $49.12_{\pm0.57}$ & $49.68_{\pm1.35}$ & $49.19_{\pm1.06}$ \\
% & VPL        
% & $49.40_{\pm0.88}$ & $49.31_{\pm0.57}$ & $49.07_{\pm0.65}$ & $48.92_{\pm0.72}$ \\
% & PAL 
% & $49.48_{\pm0.86}$ & $49.64_{\pm0.55}$ & $49.71_{\pm0.44}$ & $49.68_{\pm0.34}$ \\
% & \ours{}
% & $\textbf{96.71}_{\pm0.25}$ & $\textbf{96.21}_{\pm0.14}$ & $\textbf{97.95}_{\pm0.15}$ & $\textbf{98.19}_{\pm0.06}$ \\
% \bottomrule
% \end{tabular}
% }
% \caption{Accuracy of reward models in TL;DR.}
% \label{tab:combined_blank}
% \end{table*}


% \begin{table*}[t!]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llrrrr}
% \toprule
% && \multicolumn{2}{c}{\texttt{Gemma-2b-it}} & \multicolumn{2}{c}{\texttt{Gemma-7b-it}} \\
% \cmidrule(lr){3-4}\cmidrule(lr){5-6}
% && \multicolumn{1}{c}{ALL} & \multicolumn{1}{c}{AVG} & \multicolumn{1}{c}{ALL} & \multicolumn{1}{c}{AVG} \\
% \midrule
% \multirow{6}{*}{\rotatebox[origin=c]{90}{\emph{Seen}}}
%   & Uniform              & $62.91_{\pm0.07}$ & $62.91_{\pm0.07}$ & $63.64_{\pm0.30}$ & $63.64_{\pm0.30}$ \\
%   & I2E                  & $65.74_{\pm0.04}$ & $65.64_{\pm0.04}$ & $66.40_{\pm0.38}$ & $65.86_{\pm0.12}$ \\
%   & I2E$_{\text{proxy}}$ & $65.66_{\pm0.11}$ & $65.77_{\pm0.05}$ & $66.58_{\pm0.35}$ & $65.70_{\pm0.02}$ \\
%   & VPL                  & $70.84_{\pm0.18}$ & $67.95_{\pm0.21}$ & $70.55_{\pm0.16}$ & $66.18_{\pm0.01}$ \\
%   & PAL                  & $66.25_{\pm0.35}$ & $66.29_{\pm0.06}$ & $66.46_{\pm0.49}$ & $65.43_{\pm0.43}$ \\
%   & \textbf{CoPL}        & $\textbf{74.85}_{\pm0.17}$ & $\textbf{74.37}_{\pm0.03}$ & $\textbf{74.87}_{\pm0.19}$ & $\textbf{74.76}_{\pm0.01}$ \\
% \midrule
% \multirow{6}{*}{\rotatebox[origin=c]{90}{\emph{Unseen}}}
%   & Uniform              & $62.97_{\pm0.07}$ & $62.97_{\pm0.07}$ & $63.30_{\pm0.08}$ & $63.30_{\pm0.08}$ \\
%   & I2E                  & $65.79_{\pm0.18}$ & $66.11_{\pm0.24}$ & $65.75_{\pm0.38}$ & $65.74_{\pm0.37}$ \\
%   & I2E$_{\text{proxy}}$ & $65.49_{\pm0.10}$ & $65.79_{\pm0.04}$ & $66.47_{\pm0.08}$ & $66.13_{\pm0.33}$ \\
%   & VPL                  & $71.31_{\pm0.58}$ & $68.55_{\pm0.47}$ & $69.93_{\pm0.33}$ & $65.72_{\pm0.42}$ \\
%   & PAL                  & $65.94_{\pm0.11}$ & $66.40_{\pm0.03}$ & $66.57_{\pm0.08}$ & $65.92_{\pm0.25}$ \\
%   & \textbf{CoPL}        & $\textbf{75.69}_{\pm0.22}$ & $\textbf{75.49}_{\pm0.03}$ & $\textbf{74.84}_{\pm0.18}$ & $\textbf{75.64}_{\pm0.05}$ \\
% \bottomrule
% \end{tabular}
% }
% \caption{Accuracy of reward models in \textsc{PersonalLLM}. \textbf{Bold} marks the best result within each block. All experiments are averaged over three random seeds.}
% \label{tab:r2}
% \end{table*}
\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lllrrrrrrrr}
\toprule
&& \multicolumn{4}{c}{\texttt{Gemma-2b-it}} && \multicolumn{4}{c}{\texttt{Gemma-7b-it}} \\
\cmidrule(lr){3-6} \cmidrule(lr){8-11}
&& \multicolumn{2}{c}{TL;DR} & \multicolumn{2}{c}{PersonalLLM} && \multicolumn{2}{c}{TL;DR} & \multicolumn{2}{c}{PersonalLLM} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
&& \multicolumn{1}{c}{ALL} & \multicolumn{1}{c}{AVG} & \multicolumn{1}{c}{ALL} & \multicolumn{1}{c}{AVG} && \multicolumn{1}{c}{ALL} & \multicolumn{1}{c}{AVG} & \multicolumn{1}{c}{ALL} & \multicolumn{1}{c}{AVG} \\
\midrule
\multirow{7}{*}{\rotatebox[origin=c]{90}{\emph{Seen}}}
& Oracle   & $73.06_{\pm0.23}$ & $73.06_{\pm0.23}$ & $61.52_{\pm0.13}$ & $61.52_{\pm0.13}$ && $77.21_{\pm0.28}$ & $77.21_{\pm0.28}$ & $62.17_{\pm0.09}$ & $62.17_{\pm0.09}$ \\
\cmidrule(lr){2-11}
& Uniform  & $49.62_{\pm0.09}$ & $49.62_{\pm0.09}$ & $56.15_{\pm0.22}$ & $56.15_{\pm0.22}$ && $49.39_{\pm0.52}$ & $49.39_{\pm0.52}$ & $56.80_{\pm0.12}$ & $56.80_{\pm0.12}$ \\
& I2E      & $49.93_{\pm0.23}$ & $49.74_{\pm0.06}$ & $57.21_{\pm0.37}$ & $57.44_{\pm0.37}$ && $49.40_{\pm0.77}$ & $49.66_{\pm0.31}$ & $57.90_{\pm0.21}$ & $58.50_{\pm0.09}$ \\
& I2E$_{\text{proxy}}$
           & $49.80_{\pm0.16}$ & $49.54_{\pm0.13}$ & $56.78_{\pm0.14}$ & $57.14_{\pm0.31}$ && $49.50_{\pm0.73}$ & $49.95_{\pm0.34}$ & $57.54_{\pm0.16}$ & $58.12_{\pm0.14}$ \\
& VPL      & $49.52_{\pm0.14}$ & $49.44_{\pm0.21}$ & $56.04_{\pm1.71}$ & $56.77_{\pm0.38}$ && $49.14_{\pm0.72}$ & $49.17_{\pm0.67}$ & $58.87_{\pm0.25}$ & $57.55_{\pm1.00}$ \\
& PAL      & $50.12_{\pm0.13}$ & $50.15_{\pm0.15}$ & $56.95_{\pm0.13}$ & $57.37_{\pm0.14}$ && $49.57_{\pm0.09}$ & $49.75_{\pm0.27}$ & $57.17_{\pm0.22}$ & $56.27_{\pm0.13}$ \\
& \ours{}  & $\mathbf{96.58_{\pm0.09}}$ & $\mathbf{96.19_{\pm0.02}}$ & $\mathbf{62.57_{\pm0.38}}$ & $\mathbf{62.08_{\pm0.27}}$ && $\mathbf{97.85_{\pm0.07}}$ & $\mathbf{97.88_{\pm0.01}}$ & $\mathbf{62.90_{\pm0.05}}$ & $\mathbf{61.93_{\pm0.02}}$ \\
\midrule\midrule
\multirow{7}{*}{\rotatebox[origin=c]{90}{\emph{Unseen}}}
& Oracle   & $72.55_{\pm1.79}$ & $72.55_{\pm1.79}$ & $61.33_{\pm0.35}$ & $61.33_{\pm0.35}$ && $77.54_{\pm0.49}$ & $77.54_{\pm0.49}$ & $62.01_{\pm0.04}$ & $62.01_{\pm0.04}$ \\
\cmidrule(lr){2-11}
& Uniform  & $50.11_{\pm0.36}$ & $50.11_{\pm0.36}$ & $55.65_{\pm0.61}$ & $55.65_{\pm0.61}$ && $49.03_{\pm0.76}$ & $49.03_{\pm0.76}$ & $57.02_{\pm0.27}$ & $57.02_{\pm0.27}$ \\
& I2E      & $49.85_{\pm0.38}$ & $49.16_{\pm0.82}$ & $56.42_{\pm0.41}$ & $56.75_{\pm0.68}$ && $49.64_{\pm0.98}$ & $49.56_{\pm0.49}$ & $57.62_{\pm0.92}$ & $58.12_{\pm0.98}$ \\
& I2E$_{\text{proxy}}$
           & $49.75_{\pm0.94}$ & $49.12_{\pm0.57}$ & $56.00_{\pm1.15}$ & $56.50_{\pm0.34}$ && $49.68_{\pm1.35}$ & $49.19_{\pm1.06}$ & $57.69_{\pm0.70}$ & $57.73_{\pm0.32}$ \\
& VPL      & $49.40_{\pm0.88}$ & $49.31_{\pm0.57}$ & $54.03_{\pm1.54}$ & $56.13_{\pm0.57}$ && $49.07_{\pm0.65}$ & $48.92_{\pm0.72}$ & $58.49_{\pm1.22}$ & $56.85_{\pm0.84}$ \\
& PAL      & $49.48_{\pm0.86}$ & $49.64_{\pm0.55}$ & $57.07_{\pm0.22}$ & $57.13_{\pm0.33}$ && $49.71_{\pm0.44}$ & $49.68_{\pm0.34}$ & $57.15_{\pm0.48}$ & $56.44_{\pm0.67}$ \\
& \ours{}  & $\mathbf{96.71_{\pm0.25}}$ & $\mathbf{96.21_{\pm0.14}}$ & $\mathbf{61.62_{\pm0.10}}$ & $\mathbf{61.97_{\pm0.35}}$ && $\mathbf{97.95_{\pm0.15}}$ & $\mathbf{98.19_{\pm0.06}}$ & $\mathbf{62.77_{\pm1.32}}$ & $\mathbf{62.08_{\pm0.64}}$ \\
\bottomrule
\end{tabular}
}
\caption{Accuracy (\%) of reward models on two datasets.  
Columns labelled \textbf{TL;DR} correspond to results originally reported for UF-P-2;  
\textbf{PersonalLLM} columns correspond to UF-P-4.  
Bold numbers highlight the best method (excluding Oracle) within each \emph{Seen} or \emph{Unseen} block.  
Means $\pm$ standard deviations are computed over three random seeds.}
\label{tab:combined_tldr_personalllm}
\end{table*}



\input{table/ablation_expert_num}
